Adaptive HTAP through Elastic Resource Scheduling

Modern Hybrid Transactional/Analytical Processing (HTAP) systems use an integrated data processing engine that performs analytics on fresh data, which are ingested from a transactional engine. HTAP systems typically consider data freshness at design time, and are optimized for a fixed range of freshness requirements, addressed at a performance cost for either OLTP or OLAP. The data freshness and the performance requirements of both engines, however, may vary with the workload. We approach HTAP as a scheduling problem, addressed at runtime through elastic resource management. We model an HTAP system as a set of three individual engines: an OLTP, an OLAP and a Resource and Data Exchange (RDE) engine. We devise a scheduling algorithm which traverses the HTAP design spectrum through elastic resource management, to meet the data freshness requirements of the workload. We propose an in-memory system design which is non-intrusive to the current state-of-art OLTP and OLAP engines, and we use it to evaluate the performance of our approach. Our evaluation shows that the performance benefit of our system for OLAP queries increases over time, reaching up to 50% compared to static schedules for 100 query sequences, while maintaining a small, and controlled, drop in the OLTP throughput.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> algorithms/algo_recursive_upd_schedule.tex <==
\begin{algorithm}

\SetKwProg{Fn}{}{}{}
\SetAlgoNoLine
\DontPrintSemicolon
\SetKwFunction{isLeave}{isLeave}
\SetKwFunction{RecursiveUpd}{RecursiveUpd}%
\AlgoDisplayBlockMarkers\SetAlgoBlockMarkers{}{}%
\SetKw{Break}{break}
 \Fn{\RecursiveUpd{node}}{
%   \KwData{Some input data\\these inputs can be displayed on several lines and one
%     input can be wider than line’s width.}
%   \KwResult{Same for output data}
  %\tcc{this is a comment to tell you that we will now really start code}
  
    \If{ \isLeave{node} }{ 
        
		\eIf{node.scan == HYBRID}{
			return LOCAL
        }{
            return node.scan
        }
	}  
	\Else{	
	    node.affinity = \RecursiveUpd(node.child[1])
		\For{$i=2$ \KwTo $node.child.count$}{
		    tmp = \RecursiveUpd(node.child[i])
		    
		    \If{tmp !=  node.affinity }{
		        node.affinity = LOCAL
		        
		        \Break
		  }
		}
		\BlankLine
		return node.affinity
	}
    
}
\caption{Recursively update query schedule pseudocode}
\label{algo:update_schedule}
\end{algorithm}

==> algorithms/algo_scheduler.tex <==
\begin{algorithm}
\SetKwProg{Fn}{}{}{}
\SetKwFunction{ScheduleHTAP}{ScheduleHTAP}%
\SetKwFunction{RecursiveSetSchedule}{RecursiveSetSchedule}%
\SetKwFunction{Delta}{Delta}%
\SetKwFunction{TxnSnapshot}{TxnSnapshot}%
\SetKwFunction{isOltpElastic}{isOltpElastic}%
\SetKwFunction{QueryLocal}{QueryAnalyticalSnapshot}
\SetAlgoNoLine
\DontPrintSemicolon
\AlgoDisplayBlockMarkers\SetAlgoBlockMarkers{}{}%
\KwData{$gFrThresh$ = Freshness bound of OLAP snapshot}
\KwData{$gElasticThresh$ = Elasticity threshold}
\BlankLine
\BlankLine
 \Fn{\ScheduleHTAP{QueryPlan, $Fr_{minimum}$}}{
  \BlankLine
  \If{$Fr_{minimum}$ < $Fr_{OLAP}$}{
        return \QueryLocal{}
    }
    \BlankLine
    \TxnSnapshot{}
    \BlankLine
    \If{ \Delta{$Fr_{snapshot}$, $Fr_{OLAP}$} > $gFrThresh$ }{
        ETL()\;
        return \QueryLocal{}
    }
    \BlankLine
    
    \For{$scanAttr$ in QueryPlan}{
    
        \uIf{is relation modified}{
				scanAttr.method = LOCAL\;
		}\ElseIf{relation.hasInsertsOnly}{
		    \If{\isOltpElastic{} \&\&  reduction\_factor > $gElasticThresh$  }{
				scanAttr.method = ELASTIC\_HYBRID\;
			}\Else{
				scanAttr.method = HYBRID\;
			}
		}\Else{
			\If{\isOltpElastic{} \&\&  reduction\_factor > $gElasticThresh$  }{
				scanAttr.method = ELASTIC\_LOCAL\;
			}\Else{
			    scanAttr.method = REMOTE\;
			}
		}
    }
    
    \BlankLine
    \RecursiveSetSchedule{QueryPlan.root}\;
}

\caption{Adaptive query scheduler pseudocode}
\label{algo:query_schedule}
\end{algorithm}

==> eval_macro.tex <==
\fixme{\subsection{Per-Query Elastic Scheduling}} \label{sec:eval_marco_states}

% \begin{figure*}% >>>
%   \centering
%   \includegraphics[width=\linewidth]{eval_graphs/ch-macro-olap.pdf} 
%   \includegraphics[width=\linewidth]{eval_graphs/ch-macro-oltp.pdf} 
%   \caption
%     {%
%      ...
%       \label{fig:ch-macro}%
%     }%
% \end{figure*}% <<<

% \begin{figure*}% >>>
%   \centering
%   \subfigure[Analytical Workload]{\centering\includegraphics[width=1\linewidth]{eval_graphs/ch-macro-olap.pdf} 
%     \label{fig:ch-macro-olap}
%   }%
%   \hfill
%     \subfigure[Transactional Workload]{\centering\includegraphics[width=1\linewidth]{eval_graphs/ch-macro-oltp.pdf} 
%     \label{fig:ch-macro-oltp}
%     }%
%   \caption
%     {%
%       Hybrid OLTP and OLAP workloads under different scheduling states (PLACEHOLDER)
%       \label{fig:ch-macro}%
%     }%
% \end{figure*}% <<<

\begin{figure*}% >>>
  \centering
  \begin{minipage}[t]{.48\linewidth}
  \centering
  \subfigure[Analytical Workload]{\centering\includegraphics[width=0.8\linewidth,height=4.5cm]{eval_graphs/ch-macro-olap.pdf} 
    \label{fig:ch-macro-olap}
  }%
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{.48\linewidth}
  \centering
    \subfigure[Transactional Workload]{\centering\includegraphics[width=1\linewidth,height=4.2cm]{eval_graphs/ch-macro-oltp.pdf} 
    \label{fig:ch-macro-oltp}
    }%
  \end{minipage}%
  \caption
    {%
      Hybrid OLTP and OLAP workloads under different scheduling states
      \label{fig:ch-macro}%
    }%
\end{figure*}% <<<


Lastly, Figure~\ref{fig:ch-macro} shows the performance of both the analytical and transactional engines across the different states (S1-S3) on a subset of the  CH-benCHmark~\cite{DBLP:conf/sigmod/ColeFGGKKKNNPSSSW11}.
To evaluate RDE, we use two scan-heavy queries, Q1 \& Q6, and two join-heavy queries, Q4 \& Q19.
The tables are pre-populated according to the benchmark specification and loaded in memory.
We use a scale factor of 300 and synchronize the storage of the two engines before we start the measurements so that the OLAP engine has fresh data in the beginning of the first query.
Any subsequent snapshotting is included in the measurements.
From Q19 we remove the like condition as our engines do not support.
Figure~\ref{fig:ch-macro}(a) reports the OLAP query response times, including the data copy required for S2.
Figure~\ref{fig:ch-macro}(b) shows the OLTP throughput, including in the calculations the impact of refreshing the OLAP snapshot.
To amplify the overheads of RDE, experiments are executed run for RDE's worst case of requiring fresh data for each query, that is, each session contains exactly one query.

\textbf{Memory-bandwidth intensive.} Query 1 has high memory bandwidth requirements, as it is a filter (100\% selectivity) followed by a group-by that has a low output cardinality.
In states S2 and S3, where the OLAP engine has a local copy of the data during the actual query execution, the main performance limiter is the memory accesses for updating the local aggregates, which competes with the bandwidth to read the input data (socket-local memory bandwidth for state S2 and socket-local + interconnect bandwidth for state S3).
In addition, in state S2, the OLAP engine has to wait for the data copy to complete before starting the actual query execution.
The data copying is itself bottlenecked by the interconnect bandwidth and thus the total response time for state S2 is limited by the performance of each of the phases of the staged copying+query execution process.
When the OLAP engine is restricted to compute units that are remote to the input data (S1), the inter-connect bandwidth becomes the performance limiter.
Still, in that case, data transfer is effectively overlapped (for the 1query/sessions setup) with query execution, making the performance very similar to state S3.
State S3 is still faster as it can take advantage of the interconnect bandwidth on top of the socket-local memory bandwidth that is available to S2.
In state S2 and S3-IS the OLAP engine is not affecting the OLTP performance.
The OLAP engine is using only memory bandwidth from the OLTP socket and as our OLTP engine is store-bound, there is available bandwidth to satisfy the OLAP engine requirements.
Effectively, the RDE engine selects for this query to allocate the unused resources of the OLTP socket to increase the OLAP performance with almost zero impact on OLTP throughput.
The OLTP performance is mostly affected in state S1, where the OLTP workers running on the OLAP socket are starved in interconnect bandwidth by the OLAP engine.
Despite scaling down the OLTP engine in S3-NI, the OLTP achieves higher throughput than in state S1: the remote OLTP workers in state S1 are causing even higher interference than non-existent ones due to cross-socket atomics and congestion that end up slowing down the OLTP socket-local OLTP workers.
Overall, the RDE engine selects the state S3-NI to achieve low response time for analytics with low interference with the OLTP engine. Effectively, the RDE engine assigns the underutilized resources of the OLTP socket to the OLAP engine.

%Q4: expectation: S3 is faster as the OLAP engine has more cores and thus can hide memory latencies better.
% Catch: overfetching may end up wasting all the bandwidth, in which case this paragrah will have to change again
\textbf{Overfetching.} Query 4 joins the two biggest tables: orderline with orders. All the records of each table participate in the join, which is followed by a low output-cardinality group-by.
For demonstration purposes, we use a non-partitioned hash-join, thus the query is bounded by random accesses and memory latency during the probing phase.
In addition, the OLAP engine uses a CPU code generation backend that treats all CPU sockets as a single compute device and generates operators that handle the parallelism internally.
Thus, the join build phase of the join is intensive in atomic operations.
State S2 and S3-IS have a similar OLAP response time, as both have only intra-socket atomic operations for building the hash-table and the probing takes place in socket-local memory.
The difference in OLAP response time between S2 and S3-IS is due to the extra bandwidth (over the interconnect) available to S3-IS for reading the input data.
State S1 causes the performance of both engines to collapse as they compete for atomic over the interconnect bandwidth.
State S3-NI has a smaller slowdown compared to state S1 as in S3-NI only the OLAP engine is performing inter-socket atomic operations.
Nevertheless, S3-NI imposes a slowdown in OLAP response time, compared to S3-SI, of $\sim$20\% due the aforementioned atomic operations.
In that case RDE proposes S3-NI but as the query optimizer opts for the aforementioned join, the dynamic load balancing of the OLAP query engine abandons the OLTP-local cores and the RDE engine assigns them back to the OLTP engine.
% core All the records of each table participate in the join, which is followed by a low output-cardinality join.
% For demonstrational purposes, we use a non-partitioned hash-join, thus the query is bounded by random accesses and memory latencies during the probing phase.
% Thus, if the RDE engine wants to optimize for OLAP performance, it will increase the number of cores available to the OLAP engine by scaling it up (migrating it to state S3 and assigning it cores from the OLTP socket), the OLAP engine can issue and hide more memory requests.
% For this query, the performance of the OLTP engine degrades, as the OLAP engine is stealing both compute and memory from the OLTP side.

% Furthermore,  
% As a result, there is small interference between the OLTP and OLAP engine for state S1, S2.

\textbf{Memory-bandwidth bound.} In Q6, the analytical engine is bounded by the available bandwidth. Thus, S1 is limited by the and S2 socket-local memory bandwidth-bounded and interconnect-bounded respectively.
S3-IS takes advantage of both the local memory bandwidth as well as the interconnect bandwidth and thus achieves the combined throughput of S1 + S2. When the OLAP engine scales to the socket of the transactional engine (state S3-NI), it will start by consuming the data locally, and then the OLAP workers on the OLTP side will try to steal data from the threads that reside in the OLAP socket.
This creates a small overhead due to cache coherency and inter-socket communication and synchronization between the OLAP threads.
While the same overhead is observed in Q1, the OLAP engine executes Q6 too close to the maximum memory bandwidth, making the overhead visible for this query.

Similarly to Q1, the OLTP workload is not saturating the memory bandwidth and thus RDE can elastically scale-up the OLAP engine to the OLTP socket to reduce OLAP response times by taking advantage of the remaining memory bandwidth, without interfering with the OLTP engine.

State S3-NI is causing more interference to the OLTP engine in Q1 than Q6, due to the write to local memory for the group-by aggregates.

\textbf{Random accesses.} Q19 performs a join between a fact table (orderline) and a dimensional table (items).
The OLAP engines opts for a broadcast-based parallelization method of the join (the dimensional table is broadcasted to each OLAP worker and each worker constructs its own private hash-table, in a synchronization free manner).
The main performance limiter for the OLAP engine is random accesses during the probing phase.
State S1 that has the analytical engine accessing part of the data over the interconnect.
As a result, random accesses become even worse and race with the OLTP accesses for using the interconnect.
This has only a small effect on the transactional engine as it is store-bound.
On the other hand, the analytical engine's response time is \~4.5x higher compared to having a private copy (S2) in the OLAP socket: the increased memory latency combined with the difficulty of the code generation to vectorize and make the join probing branch-predictor-friendly are amplifying each others effect.
State S3 is improving OLAP's response time by redirecting data to the data-local cores for processing and OLAP is not competing with OLTP for interconnect resources.
The difference in execution time between state S3-IS and S3-NI is caused by the initial broadcasting phase that crosses the interconnect for S3-NI and the synchronization between the inter-socket communication and synchronization.
As for these queries the OLAP engine is bottlenecked by memory latency, RDE can migrate between the states and scale-up the analytical engine to move it closer to the fresh data, with minimal OLTP interference.


% \textbf{Random accesses.}

% explain the query sequence. which queries we support, their nature, data bound or not, how much percent data they touch usually, insert only or updates?

% Figure \ref{fig:ch-macro}. per query freshness. shows different schedules support different cases. explain each case.

% \textbf{Query sequence with maximum freshness per query.}
% ...

% \textbf{Query sequence with maximum freshness per batch.}
% ...

==> eval_macro_v1.tex <==
\subsection{Per-Query Adaptive Scheduling} \label{sec:eval_marco_states}

\begin{figure}% >>>
  \centering
  \includegraphics[width=\columnwidth]{eval_graphs/rev/ch-state-case.pdf} 
  \caption
    {%
      OLAP performance in HTAP workload under different scheduling states
     }%
     \label{fig:ch-queries-state}
\end{figure}% <<<
%\notes{idea is to create graph with sequence, for each-query.}

This section analyzes OLAP performance across different system for queries of different nature and show, how each state in our system benefits a category of OLAP queries.
% In this section, we analyze performance of four OLAP queries, CH-Q1(scan-filter-groupby), CH-Q6(scan-filter), CH-Q4(big-join), CH-Q19(fact-dimension-join), across all different states (S1-S3) of the system.

% \textbf{Methodology.} All experiments are conducted on initial database of SF300. we synchronize both, OLTP and OLAP instance, and then run OLTP-only for 10 seconds to generate fresh data. Afterwards, we execute each OLAP query 10 times for each state, and report average response time for each query.
%\revision{
\textbf{Methodology.}
We create an initial database equivalent to a scale factor of 300 and synchronize the two engines. Then we let OLTP run for 10 seconds to generate fresh data, while the OLAP engine is idle. Then we execute each query 10 times in a batch, and report average response times in Figure~\ref{fig:ch-queries-state}.

\textbf{CH-Q6 (scan-filter-reduce)} is memory intensive and its execution time highly depends on the bandwidth the OLAP engine can use to read the input.
% In State S2, all the data accessed by the OLAP engine reside in the OLAP-local socket, while in all other cases, the engine can also access 
State S2 first synchronizes the snapshot by pulling data over the interconnect and then it uses the memory bandwidth to scan data locally, restricting the performance of the OLAP engine which in any other state can combine the bandwidth, instead of having to do the consecutive scans.
%
Except S2, all states benefits from the availability of extra memory-bandwidth provided by OLTP-socket.
S1 and S3-NI are using the OLAP cores in the OLTP socket to read the local data. As the amount of elastic OLAP cores is not enough to saturate DRAM bandwidth in OLTP socket, OLAP-local cores also scan part of data over interconnect. However, in the case of S1, interconnect is shared with OLTP traffic as compared to exclusive OLAP usage in other states, hence the interference hurting performance.
%As these cores are not sufficient to saturate the available bandwidth in the OLTP-socket, cores from the other socket also scan part of the OLTP-socket-resident data.
%S1 is slower than S3-NI because remote reads interfere with the interconnect traffic generated by the OLAP-socket-resident OLTP workers.
%
S3-IS has a similar behaviour as S3-NI except that S3-IS accesses all data over interconnect. The small performance gap is due to cross-NUMA load-balancing in S3-NI, which makes elastic-cores to steal work and pull data in reverse order for reduction.

\begin{comment}% i didnt deleted this time
S3-IS has a similar behavior with S3-NI but in S3-IS all fresh data are read over the interconnect. The small performance difference between S3-IS and S3-NI is because during load balancing in S3-NI some data from the OLAP-socket are scheduled to the remote cores.
\end{comment}
%
% In State S1 and S3-NI, the OLAP engine uses 4 cores from the OLTP socket to scan local data.
% As this cores are not sufficient to saturate the available bandwidth OLAP cores from the OLAP socket are also reading data over the interconnect.
% Nevertheless, but this traffic interferes with the interconnect traffic generated by the OLTP engine.

% In states S3-IS and S3-NI . S3-IS uses the interconnect to pull remote data and directly scan them. In contrast with S1, S3-IS overlaps remote and local data scans. In S3-NI, the OLAP cores that reside in the OLTP-socket have direct access to the memory, but can not by themselves saturate the memory bandwidth. Thus, S3-NI still uses the interconnect to scan some fresh data using OLAP-socket cores. The scans over the interconnect interfere with the OLTP traffic and thus S3-NI is slightly slower than S3-IS.

\textbf{CH-Q1 (scan-filter-groupby)} is similar to Q6, but the aggregation at the end of the query has multiple groups, stressing CPU caches. Therefore, the trend in execution times is similar to Q6, however, CH-Q1 has access to more L3 cache in state S1 and S3-NI, the gap between these states closes.
%but as S1 and S3-NI increase the L3 cache accessible by the OLAP engine, the gap between them and S3-IS reduces.

\textbf{CH-Q19 (fact-dimension-join)} is a join-intensive and thus the relative cost for synchronizing the OLAP snapshot is smaller: the relative execution time of S2 is closer to the other states, as the main contributor to the execution time is the random accesses in join operation.
The OLAP engine opts for a broadcast-based join, thus S1 and S3-NI see a small performance penalty for broadcasting build-side across two NUMA nodes.
S1 gets performance hit as OLTP traffic interferes in the interconnect access. S3-NI gains over S3-IS as the broadcost is amortize by the availability of elastic-cores to OLAP engine.
%S1 is slower than S3-IS as the broadcast interferes with the OLTP traffic while both states use the same number of OLAP cores. On the other hand, for S3-NI is faster than S3-IS as the broadcast cost is overthrown by the additional cores made available to the OLAP engine.

% \textbf{CH-Q4 (big-join)}
% \vspace{1cm}% estimating space
%}

\textbf{Insights.} Per-query scheduling makes the case of adapting to nature of each query, that is, compute-bound, memory-bound or mix. Data-locality benefits memory-intensive queries and if the query is selective, data-local reduction reduces interconnect pressure in NUMA hardware. Queries with broadcast based joins, and hash-based group-by suffer from imbalanced-compute across NUMA due to cross-socket memory latencies.

\begin{comment}

Lastly, Figure~\ref{fig:ch-macro} shows the performance of both the analytical and transactional engines across the different states (S1-S3) on a subset of the  CH-benCHmark~\cite{DBLP:conf/sigmod/ColeFGGKKKNNPSSSW11}.
To evaluate RDE, we use two scan-heavy queries, Q1 \& Q6, and two join-heavy queries, Q4 \& Q19.
The tables are pre-populated according to the benchmark specification and loaded in memory.
We use a scale factor of 300 and synchronize the storage of the two engines before we start the measurements so that the OLAP engine has fresh data in the beginning of the first query.
Any subsequent snapshotting is included in the measurements.
From Q19 we remove the like condition as our engines do not support.
Figure~\ref{fig:ch-macro}(a) reports the OLAP query response times, including the data copy required for S2.
Figure~\ref{fig:ch-macro}(b) shows the OLTP throughput, including in the calculations the impact of refreshing the OLAP snapshot.
To amplify the overheads of RDE, experiments are executed run for RDE's worst case of requiring fresh data for each query, that is, each session contains exactly one query.

\textbf{Memory-bandwidth intensive.} Query 1 has high memory bandwidth requirements, as it is a filter (100\% selectivity) followed by a group-by that has a low output cardinality.
In states S2 and S3, where the OLAP engine has a local copy of the data during the actual query execution, the main performance limiter is the memory accesses for updating the local aggregates, which competes with the bandwidth to read the input data (socket-local memory bandwidth for state S2 and socket-local + interconnect bandwidth for state S3).
In addition, in state S2, the OLAP engine has to wait for the data copy to complete before starting the actual query execution.
The data copying is itself bottlenecked by the interconnect bandwidth and thus the total response time for state S2 is limited by the performance of each of the phases of the staged copying+query execution process.
When the OLAP engine is restricted to compute units that are remote to the input data (S1), the inter-connect bandwidth becomes the performance limiter.
Still, in that case, data transfer is effectively overlapped (for the 1query/sessions setup) with query execution, making the performance very similar to state S3.
State S3 is still faster as it can take advantage of the interconnect bandwidth on top of the socket-local memory bandwidth that is available to S2.
In state S2 and S3-IS the OLAP engine is not affecting the OLTP performance.
The OLAP engine is using only memory bandwidth from the OLTP socket and as our OLTP engine is store-bound, there is available bandwidth to satisfy the OLAP engine requirements.
Effectively, the RDE engine selects for this query to allocate the unused resources of the OLTP socket to increase the OLAP performance with almost zero impact on OLTP throughput.
The OLTP performance is mostly affected in state S1, where the OLTP workers running on the OLAP socket are starved in interconnect bandwidth by the OLAP engine.
Despite scaling down the OLTP engine in S3-NI, the OLTP achieves higher throughput than in state S1: the remote OLTP workers in state S1 are causing even higher interference than non-existent ones due to cross-socket atomics and congestion that end up slowing down the OLTP socket-local OLTP workers.
Overall, the RDE engine selects the state S3-NI to achieve low response time for analytics with low interference with the OLTP engine. Effectively, the RDE engine assigns the underutilized resources of the OLTP socket to the OLAP engine.

%Q4: expectation: S3 is faster as the OLAP engine has more cores and thus can hide memory latencies better.
% Catch: overfetching may end up wasting all the bandwidth, in which case this paragrah will have to change again
\textbf{Overfetching.} Query 4 joins the two biggest tables: orderline with orders. All the records of each table participate in the join, which is followed by a low output-cardinality group-by.
For demonstration purposes, we use a non-partitioned hash-join, thus the query is bounded by random accesses and memory latency during the probing phase.
In addition, the OLAP engine uses a CPU code generation backend that treats all CPU sockets as a single compute device and generates operators that handle the parallelism internally.
Thus, the join build phase of the join is intensive in atomic operations.
State S2 and S3-IS have a similar OLAP response time, as both have only intra-socket atomic operations for building the hash-table and the probing takes place in socket-local memory.
The difference in OLAP response time between S2 and S3-IS is due to the extra bandwidth (over the interconnect) available to S3-IS for reading the input data.
State S1 causes the performance of both engines to collapse as they compete for atomic over the interconnect bandwidth.
State S3-NI has a smaller slowdown compared to state S1 as in S3-NI only the OLAP engine is performing inter-socket atomic operations.
Nevertheless, S3-NI imposes a slowdown in OLAP response time, compared to S3-SI, of $\sim$20\% due the aforementioned atomic operations.
In that case RDE proposes S3-NI but as the query optimizer opts for the aforementioned join, the dynamic load balancing of the OLAP query engine abandons the OLTP-local cores and the RDE engine assigns them back to the OLTP engine.
% core All the records of each table participate in the join, which is followed by a low output-cardinality join.
% For demonstrational purposes, we use a non-partitioned hash-join, thus the query is bounded by random accesses and memory latencies during the probing phase.
% Thus, if the RDE engine wants to optimize for OLAP performance, it will increase the number of cores available to the OLAP engine by scaling it up (migrating it to state S3 and assigning it cores from the OLTP socket), the OLAP engine can issue and hide more memory requests.
% For this query, the performance of the OLTP engine degrades, as the OLAP engine is stealing both compute and memory from the OLTP side.

% Furthermore,  
% As a result, there is small interference between the OLTP and OLAP engine for state S1, S2.

\textbf{Memory-bandwidth bound.} In Q6, the analytical engine is bounded by the available bandwidth. Thus, S1 is limited by the and S2 socket-local memory bandwidth-bounded and interconnect-bounded respectively.
S3-IS takes advantage of both the local memory bandwidth as well as the interconnect bandwidth and thus achieves the combined throughput of S1 + S2. When the OLAP engine scales to the socket of the transactional engine (state S3-NI), it will start by consuming the data locally, and then the OLAP workers on the OLTP side will try to steal data from the threads that reside in the OLAP socket.
This creates a small overhead due to cache coherency and inter-socket communication and synchronization between the OLAP threads.
While the same overhead is observed in Q1, the OLAP engine executes Q6 too close to the maximum memory bandwidth, making the overhead visible for this query.

Similarly to Q1, the OLTP workload is not saturating the memory bandwidth and thus RDE can elastically scale-up the OLAP engine to the OLTP socket to reduce OLAP response times by taking advantage of the remaining memory bandwidth, without interfering with the OLTP engine.

State S3-NI is causing more interference to the OLTP engine in Q1 than Q6, due to the write to local memory for the group-by aggregates.

\textbf{Random accesses.} Q19 performs a join between a fact table (orderline) and a dimensional table (items).
The OLAP engines opts for a broadcast-based parallelization method of the join (the dimensional table is broadcasted to each OLAP worker and each worker constructs its own private hash-table, in a synchronization free manner).
The main performance limiter for the OLAP engine is random accesses during the probing phase.
State S1 that has the analytical engine accessing part of the data over the interconnect.
As a result, random accesses become even worse and race with the OLTP accesses for using the interconnect.
This has only a small effect on the transactional engine as it is store-bound.
On the other hand, the analytical engine's response time is \~4.5x higher compared to having a private copy (S2) in the OLAP socket: the increased memory latency combined with the difficulty of the code generation to vectorize and make the join probing branch-predictor-friendly are amplifying each others effect.
State S3 is improving OLAP's response time by redirecting data to the data-local cores for processing and OLAP is not competing with OLTP for interconnect resources.
The difference in execution time between state S3-IS and S3-NI is caused by the initial broadcasting phase that crosses the interconnect for S3-NI and the synchronization between the inter-socket communication and synchronization.
As for these queries the OLAP engine is bottlenecked by memory latency, RDE can migrate between the states and scale-up the analytical engine to move it closer to the fresh data, with minimal OLTP interference.

\end{comment}

==> eval_sensitivity_analysis.tex <==
\subsection{HTAP sensitivity analysis} \label{sec:eval_sensitivity_analysis}
In this section, we analyze the design states of our HTAP system and their impact on the performance of the OLTP and the OLAP engine.
We use Q1 and Q6, which perform aggregate operations over the \texttt{OrderLine} table, for two reasons: (i) they are simple queries that perform a scan over a single table, and therefore they can reveal overheads and opportunities, and, (ii) the \texttt{OrderLine} table grows in time, as the OLTP engine executes the \texttt{NewOrder} transaction.
Thus, we study the impact of data freshness-rate on the performance of both engines, at the different states that our system migrates.
We report the OLAP performance with query response time and the OLTP performance with throughput measured in million transactions per second (MTPS).
%In the following, we present our analysis for each state.

\textbf{Co-located OLTP and OLAP $\boldsymbol{[S_1]}$.}
In this state, we focus on the impact of resource allocation in the performance of each engine, due to hardware-level interference which is caused due to sharing CPU caches as well as memory and interconnect bandwidth.
We execute an experiment which considers that the engines are initially in full isolation (State $S_2$), and then they gradually trade CPUs from their sockets until they go half the way to each socket.
Both engines access the memory allocated by the OLTP engine, even though a different instance.
Therefore, initially the OLAP engine access all records from the remote socket, and it gradually gets local access as it trades its CPUs with the OLTP engine.
Instead, the OLTP engine initially has local access to its data, and gradually mixes it with remote accesses.

\begin{comment}
In this state, the OLTP and the OLAP engine share all CPU sockets available in the system.
This design is representative of the Unified Storage HTAP engine classification.
By using the two instances in OLTP, we eliminate any software-level interference, since each engine uses a separate memory area.
Instead, we focus on the impact of resource allocation in the performance of each engine, due to hardware-level interference which is caused due to sharing CPU caches as well as memory and interconnect bandwidth.
Accordingly, we execute an experiment which considers initially that the engines are in full isolation (State $S_2$), and then they gradually trade CPUs from their sockets until they go half the way to each socket, whereas they both access the memory allocated by the OLTP engine.
%Therefore, initially the OLAP engine access all records from the remote socket, and it gradually gets local access as it trades its CPUs with the OLTP engine.
%Instead, the OLTP engine initially has local access to its data, and gradually mixes it with remote accesses.
%Effectively, the number of CPUs that we trade between the two engines corresponds to the max number of CPUs that the database administrator will want to set, should this state be allowed in the system.
\end{comment}

% \begin{figure*}[t]%
%   \centering
%   \begin{minipage}[t]{.48\textwidth}
%   \centering
%   \subfigure[Co-located OLTP engine performance (higher better)]{\centering\includegraphics[width=0.8\columnwidth]{eval_graphs/trade_core-oltp.pdf} 
%     \label{fig:colocated-oltp}
%   }%
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[t]{.48\textwidth}
%   \centering
%     \subfigure[Co-located OLAP engine performance (lower better)]{\centering\includegraphics[width=0.8\columnwidth]{eval_graphs/trade_core-olap.pdf} 
%     \label{fig:colocated-olap}
%     }%
%   \end{minipage}%
%   \caption
%     {%
%       Co-located OLTP/OLAP performance (State $\boldsymbol{[S_1]}$) 
%       \label{fig:colocated-oltp-olap}%
%     }%
% \end{figure*}%

%\begin{figure*}[t]
%    \centering
%    \includegraphics[width=\textwidth]{eval_graphs/sensitivity.pdf}
%    \caption{Caption}
%    \label{fig:my_label}
%\end{figure*}

\begin{figure*}% >>>
  \centering
  \begin{minipage}[t]{.33\textwidth}
  \centering
  \subfigure[S1]{\centering\includegraphics[width=\textwidth]{eval_graphs/sensitivityS1.pdf} 
    \label{fig:sensitivityS1}
  }%
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{.33\textwidth}
  \centering
  \subfigure[S1]{\centering\includegraphics[width=\textwidth]{eval_graphs/sensitivityS2.pdf} 
    \label{fig:sensitivityS2}
  }%
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{.33\textwidth}
  \centering
  \subfigure[S1]{\centering\includegraphics[width=\textwidth]{eval_graphs/sensitivityS3NI.pdf} 
    \label{fig:sensitivityS3NI}
  }%
  \end{minipage}%
  \hfill
  \caption{Sensitivity analysis for states S1, S2, S3-NI}%
    \label{fig:sensitivityS1S2S3NI}%
\end{figure*}% <<<

\begin{figure}% >>>
  \centering
  \includegraphics[width=0.9\columnwidth,height=5cm]{eval_graphs/trade-core-oltp-olap.pdf} 
  \caption
    {%
     Co-located OLTP/OLAP perf. (State $\boldsymbol{[S_1]}$)
      \label{fig:colocated-oltp-olap}%
    }%
\end{figure}% <<<

Figure~\ref{fig:colocated-oltp-olap} shows the performance of the OLTP and the OLAP engine.
The x-axis shows the number of CPU cores traded between the engines.
The y-axis on the left-hand side of the figure shows the performance of the OLTP engine (higher is better).
The y-axis on the right-hand side of the figure shows the query response time (lower is better).
We use striped bars to represent the transactional throughput when OLTP runs without any interference from OLAP and filled bars when OLAP and OLTP are executed concurrently to depict the effect of analytical query execution to the performance of transaction execution for all configurations.
We use a line to represent the query response time.
For every configuration that we report, we run a batch of experiments where Q6 is executed 16 times, one after the other, on the freshest snapshot of data, and we report the average performance, thereby considering that the amount of fresh data in the system increases.

\begin{comment}
Figure~\ref{fig:colocated-oltp-olap} shows the performance of the OLTP and the OLAP engine as we progressively trade CPUs between the engines.
The x-axis shows the number of CPU cores traded between the engines.
The y-axis on the left-hand side of the figure shows the performance of the OLTP engine, and therefore, higher is better.
We use striped bars to represent the transactional throughput when OLTP runs without any interference from OLAP and filled bars when OLAP and OLTP are executed concurrently to depict the effect of analytical query execution to the performance of transaction execution for all configurations.
The y-axis on the right-hand side of the figure shows the query response time, and therefore, lower is better.
We use a line to represent the query response time.
For every configuration that we report, we run a batch of experiments where Q6 is executed 16 times, one after the other, on the freshest snapshot of data, and we report the average performance, thereby considering that the amount of fresh data increases.
%In every experiment, we measure the performance of the OLTP engine with and without executing OLAP in parallel, to show the effect of analytical query execution to the performance of transaction execution for all configurations.
\end{comment}

As shown in the figure, the OLTP throughput drops up to 37\% in the absence of OLAP workload execution, but after the first 4 CPUs, the rate is smaller and almost stabilizes.
This happens because the transaction execution is dominated by random memory accesses and, therefore, the interconnect does not impose much overhead.
A part of this overhead is also accounted to cross-socket atomics, as has been reported in the OLTP literature~\cite{DBLP:journals/pvldb/AppuswamyAPIA17}.
The OLTP throughput drops up to 55\% in the presence of OLAP workload execution, whereas the rate of performance degradation is almost proportional for each set of CPUs that we trade.
This is accounted to the stress caused to the memory and the interconnect bandwidth by the OLAP query, which is a scan and dominates all memory accesses.
As the OLTP moves gradually to the remote socket, it performs more accesses through the CPU interconnect which is saturated by the OLAP engine, and therefore its performance drops following this pattern.
Accordingly, we observe that the OLTP engine throughput drops about 20\% due to the interference caused by OLAP workload execution.

Similar to the OLTP throughput, we observe that the OLAP response time improves up to the point where we trade 4 CPUs, where it starts stabilizing.
The reason is that the engine efficiently load balances across the two different interconnects, memory bus and remote CPU, and pipelines execution in such a way that it does not need further data locality.
Therefore, after 4 CPUs, the OLAP performance, while the OLTP performance keeps decreasing.

\begin{comment}
Similar to the OLTP throughput, we observe that the OLAP response time improves up to the point where we trade 4 CPUs, where it starts stabilizing.
The reason is that the engine efficiently load balances across the two different interconnects, memory bus and remote CPU, and pipelines execution in such a way that it does not need further data locality.
Therefore, after 4 CPUs, the performance of the analytical query execution does not improve any further, while the performance of the OLTP engine keeps decreasing.
\end{comment}

\textbf{Insight $\boldsymbol{[S_1]}$.}
The co-location of OLTP and OLAP engine creates interference which mostly affects the performance of the OLTP engine.
Furthermore, passing many data-local CPUs to the OLAP engine does not improve its performance, whereas it continues to hurt the performance of the OLTP engine.
Therefore, a bad the decision of the topology of each engine may hurt performance with no benefit.

% \begin{figure}% >>>
%   \centering
%   \includegraphics[width=\linewidth]{eval_graphs/trade_core-olap-oltp.pdf} 
%   \caption
%     {%
%      ...
%       \label{fig:colocated-oltp-olap-single}%
%     }%
% \end{figure}% <<<

\begin{figure}% >>>
  \centering
  \includegraphics[width=0.9\columnwidth,height=5cm]{eval_graphs/etl-case.pdf} 
  \caption
    {%
     Isolated OLTP/OLAP performance (State $\boldsymbol{[S_2]}$)
      \label{fig:scan_access_path}%
    }%
\end{figure}% <<<


\textbf{Isolated OLTP and OLAP $\boldsymbol{[S_2]}$.} 
In this state, the OLTP and the OLAP engine run in their own private CPU sockets.
This design is representative of the Decoupled Storage HTAP engine classification.
Data freshness for analytical query execution is achieved by explicitly copying the snapshot of fresh data from the OLTP engine.
Therefore, the biggest overhead in this case is the time required to copy the data from one CPU socket to the other one, and how fast this cost can be amortized, by executing several queries over the same data on the OLAP socket.
Accordingly, we execute an experiment where engines do not exchange any resources, thereby keeping their original resource allocation.
We execute Q6 on the OLAP side in different batches over the same snapshot of the data.
We vary the batch size from to 1 to 16 and we transfer the fresh data from the OLTP engine before the batch execution starts.
This way, when the batch size is 1, we opt for accessing the most fresh data per query.
\revision{
On the other hand, when the batch size increases, the execution time increases and thus the accessed data become more stall as time passe. If queries in the batch are executed one after the other, then the last query in the batch accesses are less fresh.
}
We execute the same number of queries, regardless the batch size to make a fair comparison.

Figure~\ref{fig:scan_access_path} depicts the performance of the OLTP and the OLAP engine as we increase the batch size.
The x-axis shows the number of queries contained in each batch.
The y-axis on the left-hand side of the figure shows the cumulative query execution time in seconds, and therefore, lower is better.
We use solid bars to represent the response time \revision{for 16 executions of query CH-Q6 and non-solid bars to represent the time spent on transferring data between the OLTP engine and the OLAP engine, for the same 16 executions.}
The y-axis on the right-hand side of the figure shows the throughput of the OLTP engine, and therefore, higher is better.
As shown in the figure, the time required to copy the data is almost the same as the actual query execution time.
Approximately 500MB of data are copied for each batch and 160MB are accessed by each query execution.
\notes{Then why execution time is almost the same? Especially considering that the 160MB are accessed locally why the 500MB are accessed over the interconnect}.
\revision{However, as we increase the batch size, only happens once per batch and thus data copying gets amortized.}
The transactional throughput remains unaffected due to the physical isolation at the socket boundary.
The interference at the memory bus when the RDE engine copies the data to the OLAP socket does not affect the execution of transactions, since the OLTP engine does not fully utilize the memory bandwidth.

\textbf{Insight $\boldsymbol{[S_2]}$.}
Copying data from one engine to the other gets amortized after some time, provided that several queries access the same data.
Moreover, by periodically copying data to the OLAP engine, the system limits the stress on the OLTP memory bus, which is affected both when engines share their socket and when the OLAP engine reads the fresh data that it needs from the OLTP socket.
Therefore, $S_2$ brings the system into a steady state and, for this reason, the scheduler invokes it when the amount of fresh data becomes large enough.

\textbf{Hybrid OLTP and OLAP $\boldsymbol{[S_3]}$.}
In this state, the OLTP engine gives resources to OLAP and it stands in-between $S_1$ and $S_2$.
Specifically, when OLAP needs to access fresh data, it either brings them from the interconnect, or it accesses them directly by taking some CPUs of the OLTP and running in the data-local socket.
The first case, which we refer to as $S_3-IS$ (isolated), is similar to $S_2$, but the difference is that data are not copied, but only the fresh data are directly accessed from the socket where the OLTP engine is running.
Note that we cannot store the data that we bring, because this can lead to an inconsistent snapshot on the OLAP side if some records are left behind because they are not needed by the particular query.
The second case, which we refer to as $S_3-NI$ (non-isolated), is similar to $S_1$, but the difference is that the OLTP does not take any CPUs from the OLAP engine, but the latter just takes more processing.
Accordingly, the experiments that we execute measure the sensitivity of each sub-state.
\begin{figure}% >>>
  \centering
  \includegraphics[width=\columnwidth,height=4cm]{eval_graphs/fresh-data-pattern.pdf}
  \caption{OLAP response time with respect to data freshness
  \label{fig:data_pattern}}
\end{figure}% <<<

For $S3-IS$, we execute an experiment where we vary the amount of fresh data that the query will access.
We achieve this by executing Q1 for 16 times, one after the other, and requiring that it accesses fresh data.
As the OLAP engine tries to access the OLTP memory, the OLTP engine switches instance and synchronizes the two instances.
At that point, we know how many fresh records we have in the system, and we report this number.
Obviously, in this state, the analytical query execution can be easily bottlenecked by the bandwidth of the interconnect, since the OLAP will try to access all data required by the query from the remote socket.
Therefore, we optimize the access method in the plugin that our OLAP engine uses to access the data, by accessing from the remote socket only the data that are explicitly fresh.
We use this optimization only when the query accesses tables where data are \textit{inserted} and not \textit{updated}, as the latter would lead to accessing an inconsistent snapshot.
Figure~\ref{fig:data_pattern} shows the analytical query response time, as we increase the fraction of fresh data that the query accesses.
There are two important observations to be made from this plot:
(i) The default data read over the interconnect in $S_3-IS$ is worse than $S_2$, since it always has to bring the same data over the interconnect.
$S_2$ is worse in the beginning because it needs to fetch more data for the first query.
However, as we execute one query after the other, this time stabilizes;
(ii) The split-access method for $S_3$ is better because it accesses only the fresh data that are required by the query and are not stored in the socket which is local to the OLAP engine.
Moreover, we observe that the blue line of the split-access $S_3$ approaches the grey line of $S_2$, and at some point they are expected to cross.
This point is when the scheduler prefers to do the data transfer before executing the query, because most of the data is fresh.

\begin{figure}% >>>
  \centering
  \includegraphics[width=\columnwidth,height=4cm]{eval_graphs/elastic-hybrid-q1.pdf}
  \caption
    {%
      Hybrid Non-Isolated OLTP/OLAP Performance (State $\boldsymbol{[S_3-NI]}$)
      \label{fig:resource_share}%
    }%
\end{figure}% <<<

For $S_3-NI$, we vary the amount of CPUs that are passed from the OLTP to the OLAP engine.
We use Q1 for this case because Q6 introduces overheads that we explain in the following section and does not provide improvement in OLAP performance.
Effectively, this number corresponds to the maximum number of CPUs that the database administrator allows the OLAP engine to elastically expand, while sacrificing the performance of the OLTP engine.
We use the split-access method when accessing the data, since this improves the execution time.
We report the results of our experiment in Figure~\ref{fig:resource_share} which is layout similar to Figure~\ref{fig:colocated-oltp-olap}.
% The x-axis shows the number of CPU cores passed from the OLTP to the OLAP engine.
% The y-axis on the left-hand side of the figure shows the throughput of the OLTP engine, and therefore, higher is better.
% We use striped bars to represent the transactional throughput when OLTP runs without any interference from OLAP and filled bars when OLAP and OLTP are executed concurrently.
% The y-axis on the right-hand side of the figure shows the query response time, and therefore, lower is better.
% We use a line to represent the query response time.
As shown in the figure, the OLTP engine suffers from hardware-level interference, similar to the co-located case where we executed Q6.
Again, we observe that the performance of OLAP plateaus as we give it more that 6 CPUs, since it can already saturate the memory bandwidth.
The improvement that we are getting in the query response time is around 20\% in this experiment, because most of the data are accessed from the OLAP instance.

\textbf{Insight $\boldsymbol{[S_3]}$.}
We have shown that an HTAP system benefits from transferring the data from the OLTP to the OLAP side, after some freshness threshold.
Moreover, hybrid execution provides benefits to query execution, as long as there are enough data to saturate the memory bandwidth throughout the whole query execution.
Finally, we have shown the amount of resources to be passed across the engines depends on the queries and the available hardware.

==> evaluation_old.tex <==
\subsection{HTAP sensitivity analysis}
In this section, we analyze different scheduling states of OLTP and OLAP engines and there impact on performance of individual workloads. We measure OLAP performance by average query response time and OLTP performance by average transactional throughput, measured in transactions per second (TPS).

\textbf{Co-located OLTP and OLAP $\boldsymbol{[S_1]}$.}
This micro-benchmark analyzes the overheads of transactional and analytical workload when collocated in across NUMA CPU sockets. This setup uses CH-benchmark Q6, which is aggregation over \textit{orderline} relation with 100\% selectivity. In this state, the OLAP engine reads data snapshots from OLTP's inactive instance, as described in section \ref{sec:rde_engine}. Both OLTP instance, active and inactive, resides in OLTP NUMA node, and then we vary the degree of collocation of both engine to study the performance interference of hybrid workloads. Figure \ref{fig:colocated-oltp-olap} shows the experimental results when OLTP and OLAP exchange compute resources, where zero being isolated across NUMA boundaries and $14$ being, each NUMA node is allocated half to OLAP and half to OLTP engines respectively. Figure \ref{fig:colocated-oltp} shows that OLTP throughput drops by up to 37\% in the absence and up to 55\% in the presence of an analytical workload. In the absence of the OLAP query, the OLTP performance drops due to high-memory latencies of remote memory access. While on the other hand, in the presence of OLAP query, the throughput further drops as analytical query starves transactional workload on shared memory bandwidth. On the other hand, analytical workload benefits from collocation as it tends to read transactional snapshot local to the compute resource, hence overcoming NUMA interconnect bottleneck. 

\begin{figure*}% >>>
  \centering
  \begin{minipage}[t]{.48\linewidth}
  \centering
  \subfigure[Collocated OLTP Engine]{\centering\includegraphics[width=1\linewidth]{eval_graphs/trade_core-oltp.pdf} 
    \label{fig:colocated-oltp}
  }%
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{.48\linewidth}
  \centering
    \subfigure[Collocated OLAP Engine]{\centering\includegraphics[width=1\linewidth]{eval_graphs/trade_core-olap.pdf} 
    \label{fig:colocated-olap}
    }%
  \end{minipage}%
  \caption
    {%
      OLTP and OLAP performance under collocation (State $\boldsymbol{[S_1]}$), ranging from zero-core collocation to 1/2 NUMA socket OLTP and 1/2 NUMA socket OLAP. 
      \label{fig:colocated-oltp-olap}%
    }%
\end{figure*}% <<<


% \begin{figure}% >>>
%   \centering
%   \includegraphics[width=\linewidth]{eval_graphs/trade_core-olap-oltp.pdf} 
%   \caption
%     {%
%      ...
%       \label{fig:colocated-oltp-olap-single}%
%     }%
% \end{figure}% <<<

\begin{figure*}% >>>
  \centering
  \includegraphics[width=\linewidth]{eval_graphs/data-access-cases.pdf} 
  \caption
    {%
     16 query sequence (CH-Q6: 100\% selectivity) executed over varying range of freshness requirements and data access paths
      \label{fig:scan_access_path}%
    }%
\end{figure*}% <<<


\textbf{Isolated OLTP and OLAP $\boldsymbol{[S_1]}$.} 

two cases:

- When query touches major database (lineitem)

- When query touches only fraction. 

shows pros and cons, write when the cost amortizes. will put graph for Q6 and stock-level micro query


\textbf{Hybrid OLTP and OLAP $\boldsymbol{[S_3]}$.}
In this micro-benchmark, we show the benefits of elastic scheduling in terms of performance under high freshness requirements. This case is presented in two folds, state ${S_3}$-Isolated, and, ${S_3}$-NON-Isolated. 

\begin{itemize}
\item \textit{${S_3}$-Isolated}. In this schedule, the OLAP engine reads valid partial data from OLAP snapshot and additional delta from OLTP snapshot over interconnect, hence maximizing freshness while reducing the data transferred over interconnect. In this benchmark, a query sequence of sixteen query is executed while varying the number of queries executing on same snapshot. 1 query per snapshot simulates the case where each incoming query requests the maximum freshness while 16 queries per snapshot represents a query batch requesting consistent freshness across the batch. Figure \ref{fig:scan_access_path} shows the performance gain of analytical processing, through measuring cumulative query processing times, in comparison to
\begin{enumerate*}
    \item When all the data is read over interconnect, that is, remote memory scan.
    \item an ETL is performed before query execution, adding ETL latency to query latency.
\end{enumerate*}. This shows that in case of high freshness requirements, hybrid scan gives approximately same performance as accessing data from local memory at full bandwidth. However, in case of query batch, having same freshness requirement across the query bath, an ETL is preferred by paying a cost of snapshot latency which is amortized over the batch processing and also, presents the opportunity for upcoming queries to scan major portion of valid data from OLAP snapshot while querying freshness-delta over interconnect. 


\item  \textit{${S_3}$-Non-Isolated}. Under the availability of elastic OLTP resources, OLAP engine scales-out to OLTP socket in order to scan, filter and reduce data locally, utilizing the full memory bandwidth. Near-data processing benefits analytical query processing by overcoming interconnect bound data transfers and sending either reduced data or utilizing both, interconnect bandwidth to scan remote memory and memory bandwidth to scan locally over elastic compute resource. Figure \ref{fig:resource_share} shows the performance gain of analytical query when scaled-out to OLTP resources using hybrid scan while graceful throughput degradation of OLTP engine while scaling-down elastic set of resources as scheduled by the RDE engine.

\end{itemize}



% ----

% - For small amount of data, it is better to schedule query, cross boundary, but for data bound queries, interconnect is bottleneck. better do an ETL. (hybrid case will change this scenario but that is not working yet)


% \begin{figure}% >>>
%   \centering
%   \includegraphics[width=0.8\linewidth]{images/schedule_case_q1.png} 
%   \caption
%     {%
%       Hybrid and Elastic case will follow
%       \label{fig:case}%
%     }%
% \end{figure}% <<<

\begin{figure}% >>>
  \centering
  \includegraphics[width=0.8\linewidth]{images/oltp_core_alloc_sf100_q1.png} 
  \caption
    {%
      SF-100, OLTP resources allocated to OLAP to scan-local, remaining olap thread scans over interconnect. elasticity case. Input Size: 13.8GB (TO BE UPDATED with SF300 and separate OLTP and OLAP graphs)
      \label{fig:resource_share}%
    }%
\end{figure}% <<<



\subsection{Performance Opportunities}

% How input size of query and percent change of database effects the scheduling case. ETL bring all database while you might never read it..
% when ETL==remote-read, when hybrid makes difference.

% \subsection{Performance-optimized approach}

% \textbf{Near Data Processing}
% scale-down OLTP.
% \begin{itemize}
%     \item Scan-Filter-{reduce}
%         data reduction. aggregation push down before join.
% \end{itemize}


% \textbf{Mixed Scans}
% \begin{itemize}
%     \item Append-only relations.
%     Essentially, OLAP will scan the part of relation which is not update locally and the additional delta from remote. works for append-only relations.
    
%     \item{Elastic Scan} OLAP will scan somethings locally and somethings remotely.
% \end{itemize}


\textbf{Data-bound vs Compute-bound queries}
In HTAP the two engines fight for resources but at the same time each engine depending on the execution plans requires different resources, even for the the same logical plans.
For example, an analytical engine has different resource requirements for a partition-based join rather than a non-partitioned one: the partition-based join has high memory bandwidth requirements, while the non-partitioned one is restricted by latency and overfetching.
Nevertheless, selecting a memory latency-bound execution plan over a memory-bandwidth one frees up more bandwidth for the OLTP engine to proceed.

In this micro-benchmark we evaluate the behavior of the different approaches depending on the resource requirements of the analytical queries. \expected{OLAP performance depends on data locality to OLAP engine and partitioned-based joins decrease OLTP performance. As a conclusion, the optimal execution strategies for increasing the overall performance depend both on freshness requirements and analytical performance requirements. Furthermore, it may be beneficial for the overall system performance if the analytical engine selects sub-optimal plans, with respect to the analytical query latency, as long as these plans are using less resources, with a small impact on performance}




% \textbf{Joins}
% Assumption: All data in transactional snapshot ( twin-column snapshot)
% \begin{itemize}
%     \item Hash-Join
%         build local vs build remote. Racing relation-sizes. switching build relations due to sizes.
        
%     \item Index-Join:
%     as the hashtable is already present on OLTP side, twin column allows us to keep a single snapshot of index. In this case, try build side as the large relation (already have the hash-table present on primary key) and probe small relation.
% \end{itemize}


\subsection{CH-benchmark}

% \begin{figure*}% >>>
%   \centering
%   \includegraphics[width=\linewidth]{eval_graphs/ch-macro-olap.pdf} 
%   \includegraphics[width=\linewidth]{eval_graphs/ch-macro-oltp.pdf} 
%   \caption
%     {%
%      ...
%       \label{fig:ch-macro}%
%     }%
% \end{figure*}% <<<

\begin{figure*}% >>>
  \centering
  \subfigure[Analytical Workload]{\centering\includegraphics[width=1\linewidth]{eval_graphs/ch-macro-olap.pdf} 
    \label{fig:ch-macro-olap}
  }%
  \hfill
    \subfigure[Transactional Workload]{\centering\includegraphics[width=1\linewidth]{eval_graphs/ch-macro-oltp.pdf} 
    \label{fig:ch-macro-oltp}
    }%
  \caption
    {%
      Hybrid OLTP and OLAP workloads under different scheduling states (PLACEHOLDER)
      \label{fig:ch-macro}%
    }%
\end{figure*}% <<<


explain the query sequence. which queries we support, their nature, data bound or not, how much percent data they touch usually, insert only or updates?

Figure \ref{fig:ch-macro}. per query freshness. shows different schedules support different cases. explain each case.

\textbf{Query sequence with maximum freshness per query.}
...

\textbf{Query sequence with maximum freshness per batch.}
...

==> scheduling.tex <==
\section{Adaptive HTAP scheduling}
The elasticity at the system design level is driven by a scheduler which decides how to distribute resources to the OLTP and the OLAP engine.
The main parameter considered by the scheduler is the fraction of fresh data that the query is expected to access.
As execution ranges across three states: co-location, isolation, and hybrid, the scheduler requests the system to migrate to a state by changing the size of the worker pool of each engine and the affinity of the worker threads.
Accordingly, workload execution adapts to the hardware resources that are made available to the engines at every point in time.

\subsection{System model}
We model the HTAP system as a set of memory and computing resources and we assign them to the engines, which in turn use them internally to optimize their execution.
We rely on the scan operators of the analytical query plan to find the data that the query will access and we extract the fraction of fresh data.
We disregard any optimizations that may be available through the use of indices or anything related and we assume that the system will perform a full scan of each column.
Further, we assume that data are stored in a columnar layout and that there no additional overheads to scanning other than any potential NUMA effects that are caused by using CPUs that are not local to the data.
Observe that NUMA overheads are fully controllable by the scheduler, since it distributes the resources to the engines.
Finally, we assume that the database administrator can set restrictions on the amount of resources that can be revoked from the OLTP and the OLAP engine, to abide with performance guarantees and control interference between the two engines.

The main overheads that we consider in the execution are the remote memory accesses, since they can affect significantly execution times, especially in analytical query engines that have to process big amounts of data.
Given that state-of-the-art analytical query engines can saturate the memory bandwidth while scanning the data, we can quantify the overhead for remote vs local memory access to be equal to the difference in bandwidth between the main memory bus and the CPU interconnect.
For transactional engines, which are characterized by random data accesses and therefore use only a part of the memory bandwidth, we assume that the overhead for remote data access is less than the analytical ones.
Given that the profile of the transactions typically does not change over time, we assume that the scheduler can easily learn and experimentally quantify this overhead and adjust it at run-time, if the profile of the transactional workload changes.
Finally, both engines can scale as they use more CPU cores even from a socket which is remote to the data, even though bottlenecked by the interconnect, which leads to lower performance.

The scheduler makes decisions in two levels. 
The first level is the state selection.
We remind that our HTAP system has three individual states: (i) co-located OLTP and OLAP, (ii) isolated OLTP and OLAP, and, (iii) hybrid. 
The scheduler selects the state that optimizes access to the fresh data required by the query.
The second level is the resource distribution.
Memory-wise, in the co-located state, the OLTP and the OLAP engine take one of the OLTP instances each.
In the isolated case, the OLTP and the OLAP keep their own instances.
In the hybrid case, the OLTP keeps one of its active instances and shares the second with OLAP.
Computing-wise, in the co-located state, the OLTP and the OLAP share at maximum all CPU sockets.
In the isolated case, there is no change in the CPU distribution.
In the hybrid case, the OLAP engine may use a number of CPU cores that primarily belonged to the OLTP engine and interfere with its execution.
The thresholds on the amount of CPU cores to exchange between the two engines are set by the database administrator, as they affect workload execution in both engines, and therefore resource allocation has to remain compliant to any performance guarantees.

% The main invariants in HTAP scheduling are 
% \begin{enumerate*}[label=(\roman*)]
% \item Analytical and transactional processing engines are allocated with dedicated resources. In the absence of resource and data exchange, individual workload performance will be the same as the engines would run in full isolation with the same amount of resources. 
% The analytical and transactional engines itself define the performance metric, optimizing and opting for batch-throughput, tail-latency, or a compound metric, e.g., a weighted combination of throughput and latency.
% The engines itself define the performance of analytical and transactional engines, that is, the underlying engine can be either optimize and opt for batch-throughput, tail-latency or a compound performance metric, e.g., by using weights.
% \item The individual workloads would have maximum performance when executing on local resources. In the presence of resource and data exchange, either one or both systems will trade performance for analytical data freshness.
% \item Analytical data freshness is metric defined by time for the end-user, that is, by how much time the existing snapshot is stale. Moreover, it further extends to the percentage change of state of the database since the last snapshot for the underlying scheduling engine for amortizing the cost of snapshots and data-movement over time.
% \end{enumerate*}


% With the invariants mentioned above, we model the HTAP scheduler based on following global system parameters, which directs the scheduler in decision making while trading performance for analytical data freshness or vice versa.


% \begin{itemize}
    % \item \textbf{Elastic Resource Set} are the subset of dedicated resources of both analytical and transactional engines. They are marked as an elastic set of resources as an indicator for the RDE engine to elastically exchange and schedule resources, optimizing performance for given freshness levels at query-level granularity. Inherently, an elastic set of resources sets an upper-bound on performance interference of underlying hybrid workloads with each other.
    
    % \item \textbf{Minimum Freshness Guarantees} requires the scheduler to enforce minimum freshness bounds on analytical snapshots. This global parameter enables the analytical engine to answer queries in complete isolation when the required freshness is lower than the system's lower bound on freshness. Furthermore, this enforces a system to maintain freshness-bounded analytical storage to amortize the cost of snapshotting across the workloads, which have low freshness requirements \textcolor{red}{(discussed in section \ref{sec:htap_workload_classification}) : fix after fixing the ref section itself}.
% \end{itemize}

\subsection{Scheduling algorithm}

% \input{algorithms/algo_scheduler.tex}
\input{algorithms/migrate_state_s1.tex}
\input{algorithms/freshness_scheduling.tex}

Algorithm \ref{algo:query_schedule} presents the decision process involved in adaptively scheduling analytical queries with given freshness requirements and available resources. The tunable global system parameters are \emph{gFrThresh}, which is a global minimum freshness bound on OLAP snapshot, and, \emph{gElasticThresh}, which represents the global threshold for an elastic resource exchange engine. Essentially, the system only decides to elastically ship-computation near data when the incentive is higher than the global threshold. Incentive in the scope of adaptive HTAP scheduler is the data \emph{reduction factor}, that is, the factor by which the size of intermediate results would reduce before intermediate-materialization. By employing near-data processing enables the system to do efficiently schedule pipelined scan-reduce operators in order to overcome operations bottlenecked by slower interconnect bandwidth compared to local-memory bandwidth.

The scheduling algorithm greedily checks and decide to schedule the query with the goal of maximum performance and satisfying the required analytical data freshness.
The decision process starts with checking if the freshness requirement of the incoming query can be satisfied with the local OLAP snapshot; in case the query may be answered with OLAP snapshot, the query is executed, and thus, the system acts as isolated OLAP engine.

If the existing analytical snapshot cannot answer the incoming analytical query, the algorithm requests a transactional snapshot. Following the transactional snapshot, the algorithm checks the delta of freshness levels between the existing analytical snapshot and the transactional snapshot. In the event where it is greater than the global threshold \emph{gFrThresh}, the algorithm decides to initiate a complete ETL process in order to maintain minimum freshness guarantees of the system.

The primary heuristic in initiating an ETL process is, first, to guarantee minimum freshness bounds on analytical snapshots, and secondly, the ETL process is incremental, and hence, ETL latency may grow with the time since the last snapshot depending the number of distinct updates and inserts. Furthermore, it is arguable that maintain minimum-freshness bounds on analytical snapshot amortizes the cost of future queries, which will be answered by analytical snapshots only.  However, doing a periodically ETL may also not be favorable as the system might not use the analytical snapshot due to either all queries request immediate freshness or there is no analytical workload at certain time intervals.

After line 7 of algorithm \ref{algo:query_schedule}, the scheduler cannot answer queries through the existing analytical snapshot. From this point onward, the scheduler optimizes the access methods at the granularity of each attribute\footnote{attribute does not sound right word} required by the query in order to maximize performance and resource utilization while minimizing interference with the collocated transactional workload. Essentially, the scheduler has following choices to make per attribute-scan.

\begin{enumerate*}[label=(\roman*)]
\item Untouched: if the relation is untouched, that is, neither updated or inserted, then the scheduler will set the data location of the scan operator to the analytical snapshot.
\item Inserts only:  if the relation has inserts only, that is, the analytical snapshot is a subset of the transactional snapshot, then the scheduler opts for a \emph{HYBRID} scan. In \emph{HYBRID} scan, the OLAP engine reads the subset from the analytical snapshot and additional tail records from the transactional snapshot, hence utilizing local memory resources while scanning tail-records from a remote memory. Furthermore, if OLTP elastic resources are available, and the incentive of reducing data locally to the storage is greater than the \emph{gElasticThresh}, scheduler opts for \emph{ELASTIC\_HYBRID}, that is, tail records are scanned and reduced on elastic resources provided by OLTP engine.
\item Updates: if the required relation contains updated tuples since the last analytical snapshot, the scheduler has to read records from the transactional snapshot, opting for \emph{REMOTE} scan in order to guarantee consistency of snapshot across relations. In addition to \emph{REMOTE} scan, if OLTP elastic resources are available, and the incentive of reducing data locally to the storage is greater than the \emph{gElasticThresh}, scheduler opts for \emph{ELASTIC\_REMOTE}, that is, tuples are scanned and reduced on the elastic resources provided by OLTP engine. 
\end{enumerate*}

% \input{algorithms/migrate_state_s1.tex}

% \input{algorithms/algo_recursive_upd_schedule.tex}

Once the scheduler has chosen optimal access paths of each scan operation, the scheduling algorithm performs a recursive pass on the query plan, merging the execution location of query operators after scan-operation in the query plan.

Algorithm \ref{algo:update_schedule} presents the recursive-pass algorithm. It proceeds by traversing children of each operator, and if all children have the same scan affinity, the query operator is also scheduled to execute on the same computational resources. On the other hand, if the children are scheduled on both local and remote resources, the query operator is scheduled on resources local to the analytical engine in order to maximize performance and minimize performance overhead on the transactional processing.








